Heavy-heavy current improvement for calculation of $\bar{B}\rightarrow D^{(*)}\ell \bar{\nu}$ semi-leptonic form factors using the Oktay-Kronfeld action

Lattice calculations of the form factors for $\bar{B}\to D^{(*)}\ell\bar{\nu}$ decays can be used to extract the CKM matrix element $|V_{cb}|$. The Oktay-Kronfeld action is a highly improved version of the Fermilab action, which systematically reduces heavy quark discretization effects through $\mathcal{O}(\lambda^3)$ in HQET power counting, for heavy-light meson quantities. To calculate $\bar{B}\rightarrow D^{(*)}\ell \bar{\nu}$ semi-leptonic form factors using Oktay-Kronfeld heavy quarks, we need to improve the heavy quark currents to the same level. We report our progress in calculating the improvement coefficients for currents composed of bottom and charm quarks. Our results presented in this paper are preliminary.

==> matching.tex <==
\section{Matching}
\label{sec:matching_cal}

%In our recent study \cite{Bailey:2014jga}, we studied 
%two-quark matrix element with external $b$ and $c$ quark 
%and the flavor-changing operators between them.
%
%At the tree-level, the difference between continuum and
%lattice two-quark matrix element is due to difference of the 
%spinor and wave function normalization factor.
%
%By tuning the improvement parameters in the improved field,
%one can cancell out the difference.
%
%But the improvement parameters which contribute to the 
%two-quark matrix element at tree-level are only $d_1$, 
%$d_2$, $d_3$, and $d_4$, because the other parameters can 
%appear by the gluon exchange vertex.
%
%So, we need to use on-shell matrix element with at least one 
%gluon exchange to obtain constraint equations on them.

%We consider the following four-quark matrix element with 
%flavor-changing current to obtain all the improvement 
%parameters of $b$-quark up to $\mathcal{O}(\lambda^3)$,
Improvement parameters through $\mathcal{O}(\lambda^3)$
consider the following four-quark matrix  element of 
flavor-changing current,
%
\begin{align}
%\langle \ell(\eta_2, p_2) u(\eta{'}, p{'})|
\langle \ell u(\eta{'}, p{'})|
\bar{\psi}_{u}
%& \Gamma \Psi_{b} | b(\eta, p) \ell(\eta_1, p_1)\rangle_{\text{lat}},
& \Gamma \Psi_{b} | b(\eta, p) \ell \rangle_{\text{lat}},
\end{align}
%
where $\ell$ represents a light spectator quark $u$ and $b$ 
represent up quarks and bottom quarks, respectively.
%
The corresponding continuum tree-level diagrams in continuum are given 
in Fig.\ref{fig:cont-diagram_1} and 
Fig.\ref{fig:cont-diagram_2}.
%
The gluon exchange may occur at the external 
line of the $b$-quark or the $u$-quark.
%
In the case of gluon exchange at the $u$-quark line, 
however, the matching condition from the diagram is 
equivalent to that from the two-quark matrix element we 
mentioned above.
%

\begin{figure}
\centering
\subfigure[]{
\label{fig:cont-diagram_1}
\includegraphics[width=0.45\textwidth]{cont_feynman_1.jpg}
}
\subfigure[]{
\label{fig:cont-diagram_2}
\includegraphics[width=0.45\textwidth]{cont_feynman_2.jpg}
}
\caption{The tree-level, continuum diagrams for 
the four-quark matrix element with flavor-changing current.
The colored circle represents the flavor-changing operator. 
(a) The diagram with gluon exchange at the heavy-quark line.
(b) The diagram with gluon exchange at the light-quark 
line.}
\end{figure}

Therefore, the part we need to consider is the one gluon 
exchange vertex at the $b$-quark line.
%
The corresponding lattice diagrams are given in 
Fig.\ref{fig:latt-diagram_1} and 
Fig.\ref{fig:latt-diagram_2}.
%
In addition to the one-gluon exchange from the action 
vertices [Fig.\ref{fig:latt-diagram_1}] one-gluon exchange
occurs from vertices of the improvement terms in the 
quark field; the vertices are represented by dots in
Figs.\ref{fig:latt-diagram_1} and \ref{fig:latt-diagram_2}.
%
The corresponding sub-diagrams in lattice and continuum
theories are
%
\begin{align}
%
\mathcal{M}_\mu
\label{eq:matching-vertex1}
&=(-gt^a)S_b(p+q)
\gamma_\mu \sqrt{\frac{m_b}{E_b}}u_b(\eta,p)
=(-gt^a) \frac{m_b-i\gamma \cdot(p+q)}{m_b^2+(p+q)^2} \gamma_\mu 
\sqrt{\frac{m_b}{E_b}}u_b(\eta,p),
\\
\label{eq:matching-vertex2}
\mathcal{M}^{\text{lat}}_\mu
&=(-gt^a)n_\mu(q)
\Big[ R^{(0)}_b(p+q)  S^{\text{lat}}_b(p+q)\Lambda_\mu(p+q,p)
+R^{(1)}_{b,\mu}(p+q,p)\Big]
\mathcal{N}_b(p)u^{\text{lat}}_b(\eta,p),
\end{align}
%
where $q$ is the momentum of the virtual gluon and $p$ is 
the external $b$-quark momentum.
%
\begin{figure}
\centering
\subfigure[]{
\label{fig:latt-diagram_1}
\includegraphics[width=0.45\textwidth]{latt_feynman_1.jpg}
}
\subfigure[]{
\label{fig:latt-diagram_2}
\includegraphics[width=0.45\textwidth]{latt_feynman_2.jpg}
}
\caption{The tree-level, lattice diagrams with gluon exchange 
at the heavy-quark line. 
%
The dots represent (a) the zero-gluon vertex and (b) the
one-gluon vertex from the improved quark field, 
respectively.}
\end{figure}
%

\jh{The overall factor $n_\mu(q) = 2\sin \frac{1}{2}q_\mu / q_\mu 
= 1- \frac{1}{24}q_\mu^2 +\cdots$ in Eq.\eqref{eq:matching-vertex1}}
\jh{ 
is the lattice wave-function factor for gluon line.}
%
$S_b(p+q)$ and $S^{\text{lat}}_b(p+q)$ are the continuumm 
and lattice $b$-quark propagators, repectively.
%
$\mathcal{N}_b(p)$ and $u^{\text{lat}}_b(\eta,p)$ are the
lattice normalization factor and spinor of the OK action 
which correspond to continuum normalization 
$\sqrt{\frac{m_b}{E_b}}$ and spinor $u_b(\eta,p)$.
%
The one-gluon exchange vertex from action is denoted by 
$\Lambda_\mu$, and the improvement vertex with zero-gluon 
and one-gluon exchange vertex is denoted by $R^{(0)}_b$ and 
$R^{(1)}_b$, respectively.
%
\jh{The zero-gluon exchange vertex $R^{(0)}_b$ is a function of
parameter $d_1$, $d_2$, $d_3$, $d_4$,}
%
\jh{\begin{align}
&R^{(0)}(p+q) 
=e^{M_1/2} \Bigg[
1+id_1 \sum_j \gamma_j \sin(p_j +q_j) - 2d_2\sum_j \sin^2 \frac{1}{2}(p_j+q_j)
\nonumber \\
&-\frac{2}{3}i d_3 \sum_j \gamma_j \sin(p_j+q_j)\sin^2 \frac{1}{2}(p_j+q_j)
-4i d_4 \sum_{j,k}\gamma_j \sin(p_j+q_j) \sin \frac{1}{2}(p_k+q_k)
\Bigg],
\end{align}
}
\jh{where $M_1 \equiv \log(1+m_0)$ is the rest mass of 
the lattice bottom quark.}
\jh{And the temporal ($\mu=4$) and spatial ($\mu=i$) 
components of one-gluon exchange vertex $R^{(1)}_{b,\mu}$ are}
\jh{\begin{align}
&R^{(1)}_{b,4} (p+q,p)
=e^{M_1/2}\cos \frac{1}{2}q_4 \gamma_4 \Bigg[
\frac{i}{2}d_E \zeta \sum_j \gamma_j \sin q_j
-d_{EE}\gamma_4 \sum_j \gamma_j \sin q_j
\big[\sin(p_4 +q_4) - \sin(p_4)\big]
\nonumber \\
&+(d_{r_E}-d_{z_E})\sum_j \sin q_j \big[\sin(p_j+q_j)-\sin p_j \big]
-id_{r_E}\sum_{j,l,m} \epsilon_{jlm} \Sigma_j \sin q_l \big[\sin(p_m+q_m) +\sin p_m\big]
\Bigg],
\\
&R^{(1)}_{b,i}(p+q,p)
=e^{M_1/2} \Bigg[-d_1  \gamma_i \cos (p_i +\frac{1}{2}q_i)
-id_2 \sin (p_i +\frac{1}{2}q_i)
-\frac{1}{2}d_B \sum_{r,m} \epsilon_{irm} \Sigma_m \sin q_r \cos \frac{1}{2}q_i
\nonumber \\
&-\frac{i}{2}d_E \gamma_4 \gamma_i \cos \frac{1}{2}q_i \sin q_4
+d_{r_E} \sum_{r,m}i\epsilon_{irm}\Sigma_m \gamma_4 \sin q_4 \big[\sin (p_r+q_r)+\sin p_r \big] 
\cos \frac{1}{2}q_i
\nonumber \\
&-(d_{r_E}-d_{z_E})\gamma_4 \sin q_4 \big[\sin (p_i+q_i)-\sin p_i \big] \cos \frac{1}{2}q_i
+d_{EE}\gamma_i \sin q_4  
\big[ \sin(p_4 +q_4) -\sin p_4 \big]\cos \frac{1}{2}q_i
\nonumber \\
&+\frac{1}{2}d_4 
\bigg[\gamma_i \cos(p_i +\frac{1}{2}q_i)\sum_j 4\big[ \sin^2 \frac{1}{2}(p_j+q_j)
+\sin^2 \frac{1}{2}p_j \big]
+2\sin(p_i +\frac{1}{2}q_i)\sum_j \gamma_j \big[\sin(p_j +q_j) +\sin p_j \big]
\bigg]
\nonumber \\
&+\frac{1}{12}d_3 \gamma_i \bigg[4\cos(p_i +\frac{1}{2}q_i)
\big[ \sin^2 \frac{1}{2}(p_i+q_i) +\sin^2 \frac{1}{2}p_i \big]
+2\sin(p_i +\frac{1}{2}q_i) \big[\sin(p_i +q_i) +\sin p_i \big]
\bigg]
\nonumber \\
&+(d_5-d_{z_3})\cos \frac{1}{2}q_i 
\Big[-\sum_j \gamma_j \sin q_j \big[ \sin(p_i +q_i) - \sin p_i \big]
+\gamma_i \sum_j \sin q_j \big[\sin(p_j+q_j)-\sin q_j\big]\Big]
\nonumber \\
&+d_5 \cos \frac{1}{2}q_i \gamma_4 \gamma_5 \sum_{r,m}\epsilon_{irm} 
\sin q_r \big[\sin(p_m+q_m) +\sin p_m \big]
\Bigg],
\end{align}
because $p$ is on-shell momentum of bottom quark, 
$p_4 =iE_b = i\big[M_1+\frac{\boldsymbol{p}^2}{2M_2}+\cdots \big]$.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  Commented out lattice normalization and spinor %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{align}
%\mathcal{N}_b(p)u^{\text{lat}}_b(\eta,p)
%&= e^{-M_1/2}\big[ 1- \frac{i\zeta \boldsymbol{\gamma \cdot p}}{2\sinh M_1}
%-\frac{\boldsymbol{p}^2}{8M_x^2} +\frac{1}{6}iw_3 \sum_{k=1}^3 \gamma_k p_k^3
%+\frac{3i(\boldsymbol{\gamma \cdot p})\boldsymbol{p}^3}{16M_y^3}\big]
%u(\eta,0) + \mathcal{O}(\boldsymbol{p}^4)
%\\
%
%\sqrt{\frac{m_b}{E_b}}u_b(\eta,p)
%&= \Big[ 1 - \frac{i \boldsymbol{\gamma \cdot p}}{2m_b}
%-\frac{\boldsymbol{p}^2}{8m_b^2}
%+\frac{3i(\boldsymbol{\gamma \cdot p})\boldsymbol{p}^2}{16m_b^3}
%\Big]u(\eta,0) + \mathcal{O}(\boldsymbol{p}^4),
%\end{align}
%
%where $E_b = \sqrt{m_b^2 + \boldsymbol{p}^2}$ is continuum 
%energy of $b$-quark.
%
%Lattice tree-level masses $M_1$, $M_X$, $M_Y$, and the 
%rotation symmetry breaking paramter $w_3$ are functions of 
%the coefficients $r_s$, $\zeta$, $m_0$, and 
%$c_i(r_s, \zeta, m_0)$.
%
%The tree-level lattice propagator $S^{\text{lat}}_b(p+q)$ is 
%given by,
%
%\begin{align}
%S^{\text{lat}}_b(p+q)
%&= \frac{1}{i\gamma_4 \sin(p_4+q_4) 
%+ i\boldsymbol{\gamma \cdot }{\bf K}(p+q)+\mu(p+q)-\cos(p_4+q_4)}
%\nonumber\\
%&=\frac{\mu(p+q)-\cos(p_4+q_4) - i \boldsymbol{\gamma \cdot }{\bf K}(p+q)
%-i \gamma_4 \sin(p_4+q_4)}
%{\mu^2(p+q)-2\mu(p+q)\cos(p_4 +q_4) +{\bf K}^2(p+q)+1},
%\\
%\end{align}
%
%where $\text{K}_i(p+q)$ and $\mu(p+q)$ are functions of 
%momentum,
%\begin{align}
%\text{K}_i(k) &= \sin(k_i)
%\big[ \zeta -2c_2 \hat{\boldsymbol{k}}^2
%-c_1 \hat{k}^2_i \big]
%\\
%\mu(k) & = 1+m_0 + \hat{\boldsymbol{k}}^2 
%\big[\frac{1}{2}r_s \zeta +z_6 \hat{k}^2] +c_4 \sum_i \hat{k}^4_i,
%\end{align}
%where, $\hat{k}_\mu \equiv 2\sin(k_\mu/2)$.
%
%The OK action coefficient $z_6$ is zero at tree-level.
% 

Assuming that the spatial momentum $\boldsymbol{p}$ of 
external $b$-quark and the gluon momentum transfer $q$ is 
much smaller than the $b$-quark mass $m_b$ and inverse of 
the lattice spacing $1/a$, we can expand
$\mathcal{M}^{\text{lat}}_\mu$ and $\mathcal{M}_\mu$ in 
$\boldsymbol{p}a$, $qa$, $\boldsymbol{p}/m_b$, and $q/m_b$.
%
\org{For every order of $\boldsymbol{p}$ and $q$, they must
be equal.}
%
The equations at each order of $\boldsymbol{p}$ and $q$ give 
constraints on the improvement parameters $d_i$ in the 
improvement vertex $R^{(0)}$ and $R^{(1)}$.
%
Each improvement parameter $d_i$ may appear in more than one
constraint equation.
%
Parameters $d_E$, $d_{r_E}$, $d_{z_E}$, and $d_{EE}$ appear 
both in the temporal ($\mu=4$) and spatial ($\mu=i$) 
components of one-gluon exchange vertex 
$R^{(1)}_\mu$.
%
The constraint equation for $\mu=4$ and $\mu =i$ should be 
consistent.
%

For example, consider the constraint equation for the 
improvement parameter $d_{EE}$ and $\mu=4$.
%
\jh{The parameteter $d_{EE}$ contributes to matching \textit{via}
one of the terms in the one-gluon exchange vertex 
$R^{(1)}_{b,4}$.}
%
\jh{Expanding this term in the series of $\boldsymbol{p}$ and
$q$ we obtain,}
\begin{align}
-d_{EE}\cos(\frac{1}{2}q_4)\sum_j \gamma_j \sin q_j
\big[\sin(p_4 +q_4) - \sin(p_4)\big]
=-d_{EE} \cosh M_1 \boldsymbol{\gamma \cdot q}  q_4 + \cdots.
\end{align}

%
Then the lowest order constraint equation on $d_{EE}$ from 
Eq.\eqref{eq:matching-vertex1} and 
Eq.\eqref{eq:matching-vertex2},
\begin{align}
\Big[\frac{\zeta e^{-M_1}\cosh M_1}{8\sinh^3 M_1}
+\frac{\zeta c_E e^{-M_1}}{8\sinh^2 M_1}
+\frac{c_{EE}}{2\tanh M_1} -d_{EE}\cosh M_1\Big] 
\boldsymbol{\gamma \cdot q}  q_4 u(\eta,0) 
=\frac{\boldsymbol{\gamma \cdot q}  q_4 }{8m_b^3}u(\eta,0), 
\label{eq:matching-dee-temporal}
\end{align}
%
where we gathered all the linearly dependent terms at the
leading order of the Taylor expansions and equated them.
%

For the case $\mu=i$, we obtain the lowest order 
constraint equation for $d_{EE}$ in the same manner,
%
\begin{align}
\label{eq:matching-dee-spatial}
\Big[\frac{\zeta e^{-M_1}\cosh M_1}{8\sinh^3 M_1}
+\frac{\zeta c_E e^{-M_1}}{8\sinh^2 M_1}
+\frac{c_{EE}}{2\tanh M_1} -d_{EE}\cosh M_1\Big] 
  q^2_4 \gamma_i u(\eta,0) 
=\frac{1}{8m_b^3} q_4^2 \gamma_i u(\eta,0), 
\end{align}
which is exactly the same constraint on $d_{EE}$ as
Eq.\eqref{eq:matching-dee-temporal}.
%

\jh{EDIT}
We have obtained constraint equations on the all of
improvement parameters we define.
%
We have checked that all of the constraint equations are 
consistent up to the first order of $\boldsymbol{p}$.
%
And we expect $\mathcal{M}^{\text{lat}}_\mu$ and 
$\mathcal{M}_\mu$ to be matched consistently up to 
$\mathcal{O}(\boldsymbol{p}^3)$ by tuning all of the 
eleven improvement parameters,
%

The results of $d_1 - d_4$ are consistent with those
in our recent study \cite{Bailey:2014jga}, and we obtain 
newly $d_B$,
$d_{E}$, $d_{EE}$, $d_{r_E}$, $d_{z_E}$, $d_{z_3}$, and 
$d_5$ as follows,
%
\begin{align}
&d_B = d_1^2 -\frac{r_s\zeta}{2(1+m_0)}
,\\
\label{eq:result_start}
&d_E =\frac{1}{2m_b^2} 
-\frac{\zeta(1+m_0)(m_0^2+2m_0+2)}{[m_0(2+m_0)]^2}
+\frac{\zeta(1+m_0)(1-c_E)}{m_0(2+m_0)},
\\
%
&d_{r_E}=-\frac{1}{8m_b^3}+\frac{r_s\zeta}{24(1+m_0)}
+\frac{\zeta c_{EE}(2+2m_0+m_0^2)}{2m_0(1+m_0)(2+m_0)}
+\frac{\zeta^2 c_{E}(2+2m_0+m_0^2)}{[2m_0(2+m_0)]^2}   
\nonumber\\
&\quad+\frac{\zeta^2(12+24m_0 +16m_0^2+4m_0^3+m_0^4)}{12m^3_0(2+m_0)^3}
-d_1 \frac{\zeta(1+m_0)[2+m_0(2+m_0)c_E]}{2m_0^2(2+m_0)^2},
\\
%
&d_{EE} =\frac{1+m_0}{(m_0^2+2m_0+2)}\Big[-\frac{1}{4m_b^3}
+\frac{\zeta(1+m_0)(m_0^2+2m_0+2)}{[m_0(2+m_0)]^3}
\nonumber\\
&\quad+\frac{\zeta c_E(1+m_0)}{[m_0(2+m_0)]^2}
+\frac{(2+2m_0+m_0^2)c_{EE}}{m_0(2+m_0)}\Big],
\\
%
&d_5 = -\frac{1}{16m_b^3}+\frac{\zeta c_B[(1+m_0)(4+6m_0+3m_0^2)\zeta -m_0^2(2+m_0)^2d_1]}
{8(1+m_0)[m_0(2+m_0)]^2} +\frac{c_3(1+m_0)}{m_0(2+m_0)}
\nonumber\\
&\quad+\frac{\zeta^2 c_E [d_1 m_0(2+m_0) -\zeta (1+m_0)]}{4[m_0(2+m_0)]^2}
+\frac{-\zeta^2 d_1 +\zeta(1+m_0)\Big[\frac{(2+2m_0+m_0^2)\zeta^2}{[m_0(2+m_0)]^2} +d_B\Big]}
{4m_0(2+m_0)},
\\
%
& d_{z_E} = d_{z_3}=0.
\label{eq:result_end}
\end{align}

\section{Status and outstanding issues}

Results for the improvement parameters appearing in our ansatz for the improved
heavy quark field are contained in Eqs.~\eqref{eq:result_start}-\eqref{eq:result_end}.  
These results are obtained by matching the two- and four-quark flavor-changing current 
matrix elements at zeroth and first order in expansions in the momenta of the heavy
quarks.  
To simplify the matching of the four-quark matrix elements, we consider the 
$b\to u$ (heavy to light) transition instead of the $b\to c$
(heavy to heavy) transition, expand in the momentum transfer along the gluon
line, and match through second order in the momentum transfer.  

To cross-check the results in Eqs.~\eqref{eq:result_start}-\eqref{eq:result_end}, 
we have performed two sets of matching calculations.  
From the matching conditions for the two- and four-quark matrix elements, we 
find multiple independent constraints on the 11 improvement parameters. 
From these constraints we also verify that the improvement parameters in 
Eqs.~\eqref{eq:result_start}-\eqref{eq:result_end} are consistent with the
results for the improvement parameters in the OK
action~\cite{Oktay2008:PhysRevD.78.014504}.

However, several issues remain.  To summarize:  (1) Several of our results for
the improvement parameters diverge as the bare mass $m_0 \to 0$.  Since we
expect a smooth connection with the improved currents of a relativistic lattice
theory in this limit, this divergent behavior appears suspect, at least at
first glance.  (2) Although our results for $d_1$, $d_2$, and $d_B$ agree with
those in Ref.~\cite{ElKhadra:1996mp}, our result for the improvement parameter $d_E$
differs.  (3) Our matching condition yields a unique value for the improvement
parameter $d_{rE}$, even though the action operator corresponding to this
parameter is redundant.  Since the same isospectral transformations can be
applied to the action and the currents, a unique value for $d_{rE}$ indicates
the matching condition, as stated above, is incorrect.  (4) The existence of an
improved quark field corresponding to the improved currents has not been
demonstrated; the improved field can be justified, in principle, by enumerating
the HQET operators in the improved current and matching the lattice and
continuum theories order by order in
HQET~\cite{Kronfeld:PhysRevD.62.014505,Harada:2001fi,Harada:2001fj}.  These
issues may seem to invalidate the results presented in Eqs.~\eqref{eq:result_start}-\eqref{eq:result_end}.
However, such a conclusion is premature.  We note that none of these issues
represents a problem of principle.  Accordingly, we are investigating them.  

\bibliography{refs}

\end{document}

